Statistical Uncertainties of the $N_\text{DW} = 1$ QCD Axion Mass Window from Topological Defects

We review results from QCD axion string and domain wall simulations and propagate the associated uncertainties, including QCD uncertainties, into the calculation of the axion relic density. We compare two different sets of studies and, using cosmological constraints, perform statistical inference on the axion mass window in the post-inflationary Peccei-Quinn symmetry breaking scenario. For dark matter axions in recent simulations inferring a moderately infrared-dominated spectrum, this leads to a median dark matter axion mass of 0.50 meV, while the 95% credible interval at highest posterior density is between 0.48 and 0.52 meV. For alternative simulations including in addition string-domain wall decays (but with different overall inference on the spectrum), these numbers are 0.22 meV and [0.16, 0.27] meV. Relaxing the condition that axions are all of the dark matter, the axion mass window is completed by an upper bound of around 80 meV, which comes from dark radiation constraints. This confirms that the axion mass can be constrained rather precisely regarding statistical uncertainties and further calls for a more detailed analysis of the various sources of systematic uncertainties plaguing the simulations.

==> include/flowchart.tex <==
\newcommand{\drawtick}[4][0.25]{\draw[thick] ($ (#2,0) + (0,#1) $) -- ($ (#2,0) - (0,#1) $) node[below] (#3) {#4};}

\begin{tikzpicture}
	\def\TS{0.25};
	\draw[thick,-stealth] (0,0) -- (14,0) node[right] {$t$};
	\drawtick[\TS]{1}{t1}{$t_\text{ini}$};
	\drawtick[\TS]{2}{t2}{$t_\text{c}$};
	\drawtick[\TS]{7}{t3}{$t_1$};
	\drawtick[\TS]{8}{t4}{$t_2$};
	\drawtick[\TS]{9}{t5}{$t_\text{d}$};

	\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=5pt}]
	(t2) -- (t3) node [midway,yshift=-1cm] {\footnotesize Scaling regime};
	\draw[decorate,decoration={brace,amplitude=10pt,raise=1cm}]
(t3.center) -- (t4.center) node [midway,yshift=2cm] {\footnotesize DWs and strings redshift};
	
	\node[yshift=3\TS,xshift=1.5em] at (t2) {\footnotesize $T_\text{c} = \sqrt{3}\,f_a/N_\text{D}$};
	\draw[dashed,-stealth] ($ (t3) + (-1,-2) $) node[fill=white,text width=4cm,text centered] {\footnotesize DWs form,\\ realignment starts\\ $H(t_1) \sim m_a(T_1)$} -- (t3.south);
	\draw[dashed,-stealth] ($ (t4) + (3,-2) $) node[fill=white,text width=4cm,text centered] {\footnotesize DWs and strings start decaying\\ $\sigma_\text{DW} (t_2) = \xi_\text{s} (t_2)/t_2$} -- (t4.south);
\end{tikzpicture}


%\begin{tikzpicture}
%	\def\TS{0.25};
%	\draw[thick,-stealth] (0,0) -- (14,0) node[right] {$t$};
%	\drawtick[\TS]{1}{t1}{$t_\text{ini}$};
%	\drawtick[\TS]{2}{t2}{$t_\text{c}$};
%	\drawtick[\TS]{7}{t3}{$t_1$};
%	\drawtick[\TS]{8}{t4}{$t_2$};
%	\drawtick[\TS]{9}{t5}{$t_\text{d}$};
%
%	\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=5pt}]
%	(t2) -- (t3) node [midway,yshift=-1cm] {\footnotesize Scaling regime};
%	\draw[decorate,decoration={brace,amplitude=10pt,raise=1cm}]
%(t3.center) -- (t4.center) node [midway,yshift=2cm] {\footnotesize DWs and strings redshift};
%	
%	\node[yshift=3\TS,xshift=1.5em] at (t2) {\footnotesize $T_\text{c} = \sqrt{3}\,f_a/N_\text{D}$};
%	\draw[dashed,-stealth] ($ (t3) + (-1,-2) $) node[fill=white,text width=4cm,text centered] {\footnotesize DWs form,\\ realignment starts\\ $H(t_1) \sim m_a(T_1)$} -- (t3.south);
%	\draw[dashed,-stealth] ($ (t4) + (3,-2) $) node[fill=white,text width=4cm,text centered] {\footnotesize DWs and strings start decaying\\ $\sigma_\text{DW} (t_2) = \xi_\text{s} (t_2)/t_2$} -- (t4.south);
%\end{tikzpicture}
